Kayotee: A Fault Injection-based System to Assess the Safety and Reliability of Autonomous Vehicles to Faults and Errors

Fully autonomous vehicles (AVs), i.e., AVs with autonomy level 5, are expected to dominate road transportation in the near-future and contribute trillions of dollars to the global economy. The general public, government organizations, and manufacturers all have significant concern regarding resiliency and safety standards of the autonomous driving system (ADS) of AVs . In this work, we proposed and developed (a) `Kayotee' - a fault injection-based tool to systematically inject faults into software and hardware components of the ADS to assess the safety and reliability of AVs to faults and errors, and (b) an ontology model to characterize errors and safety violations impacting reliability and safety of AVs. Kayotee is capable of characterizing fault propagation and resiliency at different levels - (a) hardware, (b) software, (c) vehicle dynamics, and (d) traffic resilience. We used Kayotee to study a proprietary ADS technology built by Nvidia corporation and are currently applying Kayotee to other open-source ADS systems.

==> Makefile <==
# ACG stolen from amagela (AMA)
#This Makefile builds: congestion
#
# THE FOLLOWING TARGETS ARE GENERALLY AVAILABLE
# all:                Performs all tasks to clean, build, and install the application and documentation
# spellcheckaspell:   This runs a spell checker on all TeX files within doc/
# spellcheckhunspell: This runs a spell checker on all TeX files within doc/
# clean:              Delete the files generated from building the examples and documentation
# purge:              This does clean and also removes the resultant document
# tar:                Create a stamped, Gzip-compressed tarball within directory tar

###### USER SETTINGS ######
# TITLE:      Name of resultant documentation
TITLE:=main

###### COMPILER SETTINGS (ONLY ADMINS BELOW) ######
#COMPILERS/LINKERS
#MAKPDF:=pdflatex  --shell-escape
#MAKPDF:=pdflatex  -lualatex
MAKPDF:=latexmk -pdf
CLEAN:=latexmk -c
PURGE:=latexmk -C

SPELLCHECKTARGET:=spellcheckaspell
ifeq ($(wildcard /usr/bin/hunspell),/usr/bin/hunspell)
	SPELLCHECKTARGET:=spellcheckhunspell
endif
ifeq ($(wildcard /opt/local/bin/hunspell),/opt/local/bin/hunspell)
	SPELLCHECKTARGET:=spellcheckhunspell
endif

#EXTRA VARS
LOGAPPEND:=$(shell date '+%Y%m%d_%H%M%S')

###### TARGETS ######
default: initpurge pdf clean
#ACG perfers to call clean separately
#default: initpurge pdf
pdf: $(TITLE).pdf
$(TITLE).pdf: $(TITLE).tex
%.pdf: %.tex
#	$(MAKPDF) >$*.build.log 2>&1 $<
	$(MAKPDF) $<

.PHONY: clean
clean:
	$(CLEAN)
	-find . -type f -name "*.bbl" -exec rm -f '{}' \;
	-find . -type f -name "*~" -exec rm -f '{}' \;
	-find . -type f -name "*.swp" -exec rm -f '{}' \;
	-find . -type f -name ".*~" -exec rm -f '{}' \;
	-find . -type f -name ".*.swp" -exec rm -f '{}' \;

#ACG added to get rid of pdf but not break the other calls
#.PHONY: veryclean
#veryclean: clean
#	$(VERYCLEAN)
#	-rm $(TITLE).pdf

.PHONY: initpurge
initpurge:
	-rm -f $(TITLE).pdf

.PHONY: purge
purge: clean
	$(PURGE)

.PHONY: spellcheckaspell
spellcheckaspell:
	-find . -type f -name "[0-9]*.tex" -exec aspell -c '{}' --lang=en_US --mode=tex \;

.PHONY: spellcheckhunspell
spellcheckhunspell:
	-find . -type f -name "[0-9]*.tex" -exec hunspell -t -d en_US '{}' \;

.PHONY: spellcheck
spellcheck: $(SPELLCHECKTARGET)

.PHONY: tar
tar: clean
	mkdir -p tar
	tar -czhf tar/$(TITLE)_$(LOGAPPEND).tgz $(TITLE).pdf Makefile *.tex *.bib figs

